Computational Fluid Dynamics on 3D Point Set Surfaces

Computational fluid dynamics (CFD) in many cases requires designing 3D models manually, which is a tedious task that requires specific skills. In this paper, we present a novel method for performing CFD directly on scanned 3D point clouds. The proposed method builds an anisotropic volumetric tetrahedral mesh adapted around a point-sampled surface, without an explicit surface reconstruction step. The surface is represented by a new extended implicit moving least squares (EIMLS) scalar representation that extends the definition of the function to the entire computational domain, which makes it possible for use in immersed boundary flow simulations. The workflow we present allows us to compute flows around point-sampled geometries automatically. It also gives a better control of the precision around the surface with a limited number of computational nodes, which is a critical issue in CFD.

==> 3_point_cloud_acquisition_and_processing.tex <==
%-------------------------------------------------------------------------------%
% Section: Point cloud acquisiton and processing
%-------------------------------------------------------------------------------%
\section{Point cloud acquisition and processing}
\label{sec:point_cloud_acquisition_and_processing}

%-------------------------------------------------------------------------------%
\subsection{Datasets}

\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{../schemas/datasets_3d.jpg}
	\caption{The four 3D datasets used in this article. (a) a synthetic point cloud made out from a CAD box model. (b) The Stanford Bunny 3D scanned from a clay statue. (c) Saint Jacques meeting room at the school of Mines. (d) Portion of Madame street in Paris \todo[inline]{A completer + prendre ne photo plus jolie de la salle Saint Jacques + quid des droits d'images pour le scanner Cyberware ?}}  
	\label{fig:datasets_3d}
\end{figure}

3D scanning techniques enable us to make 3D models from real-life objects. Nowadays, they are widely used for both industrial and consumers applications. The 3D measurement can be performed thanks to various physical phenomenon : contact scanners uses the resistive force of a surface, laser scanners uses the Lambertian reflectivity of a surface to measure the time of flight of a laser beam shooted hundred of thousands times per second, CT scans and other related volumetric scanners can produce 3D slices of an object. In this work we will focus only on surface 3D scanning techniques. \cite{zhao_direct_2016} present the same adaptive finite element simulation framework on volumetric data.

In order to illustrate our work, we chose 4 different point cloud datasets depicted in Figure~\ref{fig:datasets_3d}:
\begin{enumerate}[label=(\alph*)]
	\item \textbf{box}: This is a synthetic point cloud made out from a CAD box model. Its dimensions are: \todo{Put dimensions here}. And it is composed of \todo{Add point number here} 3D points uniformly sampled on the surface. The results for this synthetic dataset will be later compared to well known benchmarks in CFD.
	
	\item \textbf{bunny}: This dataset have been acquired by the Stanford University Computer Graphics Laboratory in 1993-4. It has been scanned thanks to a Cyberware 3030 MS scanner from a clay statue. \todo[inline]{Acquisition process(nb scans ...) + registration + geometric characteristics + well known point cloud in the community + characteristics: nb pts...}
	
	\item \textbf{room}: Saint Jacques room is a meeting room in the main building of the school of Mines in Paris. This room has ancient brick walls and a dome ceiling. It has been acquired thanks to a Faro Focus X130 3D Terrestrial Laser Scanner (TLS). The mean local accuracy of each scan is 2mm. 5 scan have been acquired in various positions in the room. They have been registered thanks to an ICP-based algorithm \cite{rusinkiewicz_efficient_2001}
	\todo[inline]{geometric characteristics + characteristics: nb pts...}
	
	\item \textbf{street}: The Madame street is located in the 6th Parisian district. It is a public available dataset for point cloud segmentation and classification \cite{serna_paris-rue-madame_2014}. It have been acquired by L3D2 prototype of the CAOR robotics laboratory of the school of Mines which is a Mobile Mapping System (MMS) \cite{goulette_integrated_2006}. It is equipped with and INS/GPS localization system and a Velodyne HDL32E lidar. This latter has an accuracy of 2cm and its 32 laser beams mouted on a 10Hz spinning head produce up to 700,000 point per second. An MMS is designed to acquire urban 3D data with high productivity rate, as the vehicles moves at normal speed in the traffic.
	\todo[inline]{geometric characteristics + characteristics: nb pts...}
\end{enumerate}

As it was said before, these datasets have been chosen to cover a wide range of 3D scanning techniques. This choice has also been motivated by specific CFD applications, trying to cover a wide range of industrial usages. Each simulation test case will be described later in the Section \ref{sec:results} later in this article.


%-------------------------------------------------------------------------------%
\subsection{Point cloud preprocessing}

Preprocessing pipeline: \todo{Ajouter references pour chaque partie}

\subsubsection*{Outliers removal}

\todo[inline]{Parler du bruit structur\'{e} qui peut etre complexe a retirer (par exemple aux abords d'une table dans un scan fixe)}

\subsubsection*{Segmentation} Some part of the dataset must be removed (and eventually replaced by other representation, e.g: trees), or some part must be automatically identified in order to enforce different boundary conditions. Here only manual segmentation is automatic segmentation can also be used.

\subsubsection*{Subsampling}

\todo[inline]{Citer article CloudCompare sur octree + citer dautres papiers plus complexes style Interactive Editing of Large Point Clouds(Wand) etc...}

\subsubsection*{Normals computing}



==> _immersed_boundary_simulation.tex <==
\section{Immersed boundary flow simulation}
\label{sec:immersed_boundary_flow_simulation}

%-------------------------------------------------------------------------------%
\subsection{Related work}
\noindent \hl{[Partir de }\cite{mittal_immersed_2005} ?\hl{ [Regarder dans Zotero la collection d'articles] [Redondance avec l'etat de l'art donne plus haut en introduction ?]}

\noindent \hl{[Pas possible d'etre exhaustif -> Mettre uniquement en evidence les enjeux et la philosophie qui se degagent des principales methodes (ex : les premieres methodes se faisaient sur des grilles regulieres et que pas mal de travail a ete mis en oeuvre pour palier aux problemes aux frontieres + les premieres methodes etaient plutot faites pour l'interaction fluide-structure)]}


%-------------------------------------------------------------------------------%
\subsection{New formulation from the dirac function}

\noindent \hl{[Titre a modifier]}

\noindent \hl{[Resumer les principaux resultats 2D de l'article de Simon]}

\noindent \hl{[Insister sur le fait qu'on peut calculer la force qui s'applique sur l'obstacle directement avec cette methode]}

